Dimers and M-Curves

In this paper we develop a general approach to dimer models analogous to Krichever's scheme in the theory of integrable systems. We start with a Riemann surface and the simplest generic meromorphic functions on it and demonstrate how to obtain integrable dimer models. These are dimer models on doubly periodic bipartite graphs with quasi-periodic positive weights. Dimer models with periodic weights and Harnack curves are recovered as a special case. This generalization from Harnack curves to general M-curves leads to transparent algebro-geometric structures. In particular explicit formulas for the Ronkin function and surface tension as integrals of meromorphic differentials on M-curves are obtained. Furthermore we describe the variational principle for the height function in the quasi-periodic case. Based on Schottky uniformizations of Riemann surfaces we present concrete computational results including computing the weights and sampling dimer configurations with them. The computational results are in complete agreement with the theoretical predictions.

==> Sections/11_RonkinFunctionViaSchottky.tex <==
\section{Ronkin function via Schottky data}
\label{sec:11_Ronkin_function_via_Schottky}

{\AB{
\begin{itemize}
\item AB and NB will check
\item $g=0$ case. Derivation of the formulas for Ronkin and dual Ronkin (free energy and surface tension) in terms of dilogarithms
\item $g=g$ case. (Dream!) Ronkin function as averaging of the $g=0$ Ronkin function over the Schottky group 
\end{itemize}
}}

\NB{
	\begin{itemize}
		\item Use real line as $X_0$.
		\item $g=0$. $\alpha, \beta, \gamma = 0,1,\infty$ gives Kenyon formula for $\sigma$
		\item $g=0$. Square lattice formula for $\sigma$ depending on $cr(\alpha^-, \beta^-, \alpha^+, \beta^+)$.
		\item $g=g$. Factorization into dual group elements for real structure.
	\end{itemize}
}



==> Sections/PrymReductions.tex <==
\section{Prym reductions}

The real reduction (discussed here for $M$-curves) is compatible with the two-sheeted covering reduction. 

Assume that $\mathcal{R}$ possesses, apart from an anti-holomorphic involution $\tau$, a commuting holomorphic involution $\pi$ without fixed points. One can assume that $\pi X_0=X_0$. Grushevsky-Krichever demonstrated that, in the case of a regular square lattice and $\alpha_i^-=\pi\alpha_i^+$, $\beta_i^-=\pi\beta_i^+$, the Baker-Akhiezer functions from the kernel of the 4-point Dirac operator are gauge equivalent to solutions of the so called \emph{Moutard equation} $\psi_{m+1,n+1}-\psi_{m,n}=u_{m,n}(\psi_{m,n+1}-\psi_{m+1,n})$ with the purely imaginary potentials $u_{m,n}$. In the case $g=1$, so that $g(\mathcal{R}/\pi)=1$ and $\dim \text{Prym}(\mathcal{R})=0$, we arrive at the local Dirac operators from our previous paper (note that the corresponding Moutard potential are non-local). In the higher genus situation, everything becomes non-local. 

A similar construction with a two-sheeted ramified covering, when $\pi$ has two fixed points, was considered by Doliwa et al. Here the simplest situation is
$g=2$, so that $g(\mathcal{R}/\pi)=1$ and $\dim \text{Prym}(\mathcal{R})=1$.
